Hypergraph-Regularized Gramian Volumes for Multimodal Retrieval

Volume-based multimodal retrieval jointly scores a text query with a candidate's video, audio, and subtitle embeddings. While this approach captures higher-order within-candidate alignment, the score remains candidate-local, and semantically related training samples primarily serve as contrastive negatives. This work introduces Hypergraph-Regularized Gramian Volumes (HyVol), a training-time module that incorporates these semantic relations prior to evaluating the original volume loss. Document hyperedges connect the observed modalities of each candidate, whereas semantic hyperedges link candidates whose detached captions are mutual top-k neighbors. A shallow gated hyper-graph network applies residual corrections to the modality embeddings. Presence masks exclude unavailable streams from message passing, and identity padding preserves the determinant of the observed Gram submatrix without feature imputation. As refinement operates on embeddings rather than scores, the same construction applies to both Gram and HyperGram. We remove the hypergraph after training, leaving the backbone-only architecture, original scoring function, and retrieval cost unchanged. We train both backbones on a 150K-clip subset of VAST-27M and evaluate zero-shot performance on six benchmarks. Under the paired protocol, HyVol improves R@1 across all five retrieval benchmarks, with video-to-text gains reaching +8.3 on MSR-VTT and +7.6 on VATEX. Under missing-modality masking, the V2T margin remains positive in all experimental settings, although the T2V margin becomes slightly negative in four.

==> Tables/Implementation_Details.tex <==
\begin{table}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.15}
\caption{\hyvol hyperparameters.}
\label{tab:hparams}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}llr@{}}
\toprule
Group & Hyperparameter & Value \\
\midrule
\multirow{5}{*}{Hypergraph}
 & neighbours $k$ (\texttt{knn\_k})         & $12$ \\
 & adaptive cap $\lfloor B/4\rfloor$         & $16$ \\
 & edge dropout $p_{\mathrm{drop}}$          & $0.3$ \\
 & similarity floor $\sigma_{\mathrm{std}}$  & disabled \\
 & semantic edges                            & train only \\
\midrule
\multirow{3}{*}{Edge attention}
 & feature dim $K$                           & $512$ \\
 & LeakyReLU slope                           & $0.2$ \\
 & $\mathbf{a}$ init                         & $\mathcal{N}(0,0.1^2)$ \\
\midrule
\multirow{3}{*}{GatedHGNN}
 & layers $L$                                & $2$ \\
 & gate init $g_l$                           & $1.0$ \\
 & activation                                & GELU \\
\midrule
\multirow{4}{*}{Loss}
 & temperature $\tau$ (learned)              & $0.07$ \\
 & label smoothing                           & $0.1$ \\
 & doc weight $w_{\mathrm{doc}}$             & $1.0$ \\
 & variance weight $w_{\mathrm{reg}}$        & $0.1$ \\
\midrule
\multirow{7}{*}{Training}
 & encoder lr $\eta$                         & $2\times10^{-5}$ \\
 & graph lr $\eta_{\mathrm{graph}}$          & $5\times10^{-4}$ \\
 & global batch $B$                          & $256$ \\
 & \quad per GPU ($\times4$)                 & $64$ \\
 & epochs / frames                           & $1$ / $2$ \\
 & audio per clip                            & one $10$\,s clip \\
 & precision                                 & fp16 (graph fp32) \\
\bottomrule
\end{tabular*}
\end{table}

==> Tables/main_results4.tex <==
\begin{table*}[t]
\centering
\caption{
Effect of the number of retrieved candidates $K$ in \hyvol, applied on top of GRAM (HHR-GRAM).
R@1 is reported for all benchmarks; AudioCaps reports text-to-audio R@1
and VGGSound-5K reports audio--text classification Acc@1.
}
\label{tab:topk_ablation}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lc cccc cccc@{}}
\toprule
\multirow{2}{*}{Benchmark}
& \multirow{2}{*}{Modalities}
& \multicolumn{4}{c}{Text $\rightarrow$ Video (R@1)}
& \multicolumn{4}{c}{Video $\rightarrow$ Text (R@1)} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & $K{=}4$ & $K{=}8$ & $K{=}12$ & $K{=}16$
  & $K{=}4$ & $K{=}8$ & $K{=}12$ & $K{=}16$ \\
\midrule
\multirow{3}{*}{MSR-VTT}
& T--V   & 50.0 & 52.1 & \textbf{52.6} & 51.1 & 47.7 & 52.2 & \textbf{54.5} & 54.4 \\
& T--VA  & 50.6 & 52.5 & \textbf{54.0} & 52.1 & 49.0 & 51.8 & \textbf{55.8} & 55.7 \\
& T--VAS & 53.2 & 54.3 & \textbf{55.8} & 54.7 & 51.9 & 53.7 & \textbf{58.1} & 57.6 \\
\midrule
\multirow{2}{*}{DiDeMo}
& T--V  & 50.0 & 51.8 & \textbf{53.8} & 52.5 & 48.0 & 52.6 & \textbf{53.8} & \textbf{53.8} \\
& T--VA & 50.3 & 51.4 & \textbf{54.6} & 52.4 & 48.4 & 52.7 & \textbf{54.1} & 53.3 \\
\midrule
\multirow{2}{*}{ActivityNet}
& T--V  & 53.3 & 55.9 & \textbf{56.2} & 54.9 & 47.8 & 50.6 & \textbf{56.2} & 49.2 \\
& T--VA & 53.9 & 56.7 & \textbf{56.9} & 55.4 & 48.4 & 50.2 & \textbf{56.6} & 49.8 \\
\midrule
\multirow{3}{*}{VATEX}
& T--V   & 87.7 & 91.9 & \textbf{92.1} & 91.9 & 91.4 & 92.1 & \textbf{92.3} & 91.6 \\
& T--VA  & 89.0 & 91.9 & 93.0 & \textbf{93.3} & 91.7 & 92.1 & \textbf{92.8} & 92.3 \\
& T--VAS & 90.1 & 92.6 & \textbf{94.0} & 93.5 & 93.3 & 93.7 & \textbf{93.8} & 93.0 \\
\midrule
AudioCaps
& T--AV & 32.0 & 35.5 & \textbf{35.7} & 35.2 & -- & -- & -- & -- \\
VGGSound-5K
& T--AV & 39.7 & \textbf{40.9} & \textbf{40.9} & 40.4 & -- & -- & -- & -- \\
\bottomrule
\end{tabular*}
\end{table*}
